To be or not to be: Roughness or long memory in volatility?

We develop a framework for composite likelihood estimation of parametric continuous-time stationary Gaussian processes. We derive the asymptotic theory of the associated maximum composite likelihood estimator. We implement our approach on a pair of models that have been proposed to describe the random log-spot variance of financial asset returns. A simulation study shows that it delivers good performance in these settings and improves upon a method-of-moments estimation. In an empirical investigation, we inspect the dynamic of an intraday measure of the spot log-realized variance computed with high-frequency data from the cryptocurrency market. The evidence supports a mechanism, where the short- and long-term correlation structure of stochastic volatility are decoupled in order to capture its properties at different time scales. This is further backed by an analysis of the associated spot log-trading volume.

==> tables/sim-mcle-cc-q=2-N=1-mu=0.tex <==
\begin{sidewaystable}[ht!]
\setlength{ \tabcolsep}{0.15cm}
\begin{center}
\caption{Parameter estimation of the Cauchy class [$q = 2$ and $\mu$ known].}
\label{table:sim-cc-q=2-N=1-mu=0}
\begin{footnotesize}
\begin{tabular}{lrrrrrrrrrrrrrr}
\hline \hline
Parameter & Value & \multicolumn{3}{c}{$T = 1{,}095$} && \multicolumn{3}{c}{$T = 1{,}825$} && \multicolumn{3}{c}{$T = 2{,}555$} \\
\cline{3-5} \cline{7-9} \cline{11-13}
&& \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} && \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} && \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} \\
\hline 
Panel A: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\beta$ & 0.250 & 0.144 (0.334) & 0.052 (0.183) & 1.878 & & 0.112 (0.240) & 0.017 (0.155) & 1.625 & & 0.095 (0.202) & -0.005 (0.141) & 1.512 \\
$\nu$ & 1.250 & -0.001 (0.075) & -0.001 (0.075) & 1.002 & & -0.001 (0.068) & -0.001 (0.068) & 1.001 & & -0.001 (0.064) & -0.001 (0.064) & 1.001 \\
$\alpha$ & -0.450 & 0.019 (0.050) & -0.020 (0.028) & 1.644 & & 0.015 (0.036) & -0.024 (0.022) & 1.342 & & 0.012 (0.030) & -0.026 (0.019) & 1.169 \\
Panel B: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\beta$ & 0.500 & 0.095 (0.322) & -0.124 (0.203) & 1.486 & & 0.064 (0.231) & -0.149 (0.178) & 1.139 & & 0.050 (0.192) & -0.163 (0.164) & 0.971 \\
$\nu$ & 0.750 & -0.000 (0.026) & -0.000 (0.026) & 1.003 & & -0.000 (0.021) & -0.000 (0.021) & 1.002 & & -0.000 (0.018) & -0.000 (0.018) & 1.002 \\
$\alpha$ & -0.400 & 0.015 (0.056) & -0.063 (0.032) & 1.038 & & 0.010 (0.040) & -0.067 (0.026) & 0.761 & & 0.008 (0.033) & -0.068 (0.023) & 0.631 \\
Panel C: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\beta$ & 0.750 & 0.047 (0.208) & -0.058 (0.123) & 1.619 & & 0.028 (0.155) & -0.063 (0.097) & 1.466 & & 0.020 (0.129) & -0.067 (0.088) & 1.300 \\
$\nu$ & 0.500 & -0.000 (0.018) & -0.000 (0.018) & 1.003 & & -0.000 (0.014) & -0.000 (0.014) & 1.002 & & -0.000 (0.012) & -0.000 (0.012) & 1.001 \\
$\alpha$ & -0.200 & 0.014 (0.069) & -0.170 (0.045) & 0.541 & & 0.008 (0.051) & -0.169 (0.035) & 0.414 & & 0.006 (0.042) & -0.168 (0.030) & 0.347 \\
Panel D: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\beta$ & 1.000 & 0.049 (0.238) & -0.117 (0.105) & 1.800 & & 0.028 (0.172) & -0.126 (0.088) & 1.391 & & 0.020 (0.142) & -0.130 (0.079) & 1.173 \\
$\nu$ & 0.300 & -0.000 (0.010) & -0.000 (0.010) & 1.003 & & -0.000 (0.008) & -0.000 (0.008) & 1.002 & & -0.000 (0.006) & -0.000 (0.006) & 1.001 \\
$\alpha$ & 0.000 & 0.020 (0.105) & -0.259 (0.044) & 0.560 & & 0.011 (0.076) & -0.258 (0.034) & 0.412 & & 0.008 (0.063) & -0.258 (0.029) & 0.341 \\
Panel E: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\beta$ & 1.250 & 0.057 (0.278) & -0.196 (0.115) & 1.562 & & 0.040 (0.220) & -0.202 (0.092) & 1.307 & & 0.030 (0.186) & -0.204 (0.080) & 1.135 \\
$\nu$ & 0.200 & -0.000 (0.006) & -0.000 (0.006) & 1.002 & & -0.000 (0.005) & -0.000 (0.005) & 1.002 & & -0.000 (0.004) & -0.000 (0.004) & 1.001 \\
$\alpha$ & 0.200 & 0.027 (0.139) & -0.349 (0.042) & 0.562 & & 0.019 (0.113) & -0.348 (0.033) & 0.457 & & 0.015 (0.096) & -0.348 (0.027) & 0.392 \\
\hline \hline
\end{tabular}
\end{footnotesize}
\smallskip
\begin{scriptsize}
\parbox{0.98\textwidth}{\emph{Note.} 
We simulate the process in the caption of the table 10,000 times on the interval $[0,T]$, where $T$ is interpreted as the number of days. 
There is $N = 1$ observation per unit interval, corresponding to one every day.
The true value of the parameter vector appears to the left in Panel A -- E. 
We estimate $\theta$ with the maximum composite likelihod estimation (MCLE) procedure developed in the main text, and benchmark it against a method-of-moments estimator (MME).
The table shows the Monte Carlo average of each parameter estimate across simulations (standard deviation in parenthesis).
The last column reports the RMSE ratio defined as $\text{RMSE}_{r} = \text{RMSE}( \hat{ \theta}_{ \text{MCLE}}) / \text{RMSE}( \hat{ \theta}_{ \text{MME}})$. 
}
\end{scriptsize}
\end{center}
\end{sidewaystable}


==> tables/sim-mcle-cc-q=2-N=1-mu=1.tex <==
\begin{sidewaystable}[ht!]
\setlength{ \tabcolsep}{0.15cm}
\begin{center}
\caption{Parameter estimation of the Cauchy class [$q = 2$ and $\mu$ estimated].}
\label{table:sim-cc-q=2-N=1-mu=1}
\begin{footnotesize}
\begin{tabular}{lrrrrrrrrrrrrrr}
\hline \hline
Parameter & Value & \multicolumn{3}{c}{$T = 1{,}095$} && \multicolumn{3}{c}{$T = 1{,}825$} && \multicolumn{3}{c}{$T = 2{,}555$} \\
\cline{3-5} \cline{7-9} \cline{11-13}
&& \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} && \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} && \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} \\
\hline 
Panel A: \\
$\mu$ & 0.000 & 0.005 (0.361) & 0.005 (0.361) & 1.001 & & 0.004 (0.346) & 0.004 (0.345) & 1.001 & & 0.004 (0.336) & 0.004 (0.336) & 1.001 \\
$\beta$ & 0.250 & 0.411 (0.425) & 0.204 (0.196) & 2.115 & & 0.339 (0.282) & 0.153 (0.164) & 1.881 & & 0.296 (0.218) & 0.125 (0.150) & 1.735 \\
$\nu$ & 1.250 & -0.053 (0.029) & -0.053 (0.029) & 1.002 & & -0.048 (0.024) & -0.048 (0.024) & 1.001 & & -0.046 (0.021) & -0.046 (0.021) & 1.001 \\
$\alpha$ & -0.450 & 0.049 (0.068) & -0.020 (0.028) & 2.433 & & 0.042 (0.044) & -0.024 (0.022) & 1.900 & & 0.037 (0.034) & -0.026 (0.019) & 1.608 \\
Panel B: \\
$\mu$ & 0.000 & 0.002 (0.140) & 0.002 (0.140) & 1.003 & & 0.002 (0.127) & 0.002 (0.127) & 1.002 & & 0.002 (0.119) & 0.002 (0.119) & 1.001 \\
$\beta$ & 0.500 & 0.279 (0.366) & -0.013 (0.204) & 2.033 & & 0.210 (0.246) & -0.047 (0.176) & 1.607 & & 0.173 (0.195) & -0.067 (0.162) & 1.361 \\
$\nu$ & 0.750 & -0.013 (0.019) & -0.013 (0.018) & 1.002 & & -0.011 (0.015) & -0.011 (0.015) & 1.002 & & -0.010 (0.013) & -0.010 (0.013) & 1.001 \\
$\alpha$ & -0.400 & 0.040 (0.066) & -0.063 (0.032) & 1.312 & & 0.030 (0.044) & -0.067 (0.026) & 0.911 & & 0.025 (0.035) & -0.068 (0.023) & 0.733 \\
Panel C: \\
$\mu$ & 0.000 & 0.000 (0.078) & 0.000 (0.077) & 1.004 & & 0.001 (0.065) & 0.001 (0.065) & 1.003 & & 0.001 (0.058) & 0.001 (0.058) & 1.002 \\
$\beta$ & 0.750 & 0.141 (0.218) & 0.026 (0.108) & 2.182 & & 0.091 (0.155) & 0.011 (0.077) & 2.167 & & 0.069 (0.128) & 0.002 (0.064) & 2.150 \\
$\nu$ & 0.500 & -0.006 (0.016) & -0.006 (0.016) & 1.002 & & -0.004 (0.013) & -0.004 (0.013) & 1.002 & & -0.004 (0.011) & -0.004 (0.011) & 1.001 \\
$\alpha$ & -0.200 & 0.040 (0.072) & -0.170 (0.045) & 0.602 & & 0.025 (0.051) & -0.169 (0.035) & 0.437 & & 0.019 (0.042) & -0.168 (0.030) & 0.363 \\
Panel D: \\
$\mu$ & 0.000 & 0.000 (0.032) & 0.000 (0.032) & 1.005 & & 0.000 (0.026) & 0.000 (0.025) & 1.003 & & 0.000 (0.022) & 0.000 (0.022) & 1.002 \\
$\beta$ & 1.000 & 0.113 (0.252) & -0.051 (0.084) & 2.892 & & 0.066 (0.177) & -0.073 (0.068) & 2.150 & & 0.048 (0.144) & -0.084 (0.060) & 1.754 \\
$\nu$ & 0.300 & -0.002 (0.010) & -0.002 (0.010) & 1.002 & & -0.001 (0.007) & -0.001 (0.007) & 1.002 & & -0.001 (0.006) & -0.001 (0.006) & 1.001 \\
$\alpha$ & 0.000 & 0.044 (0.110) & -0.259 (0.044) & 0.604 & & 0.025 (0.078) & -0.258 (0.034) & 0.429 & & 0.018 (0.064) & -0.258 (0.029) & 0.352 \\
Panel E: \\
$\mu$ & 0.000 & 0.000 (0.016) & 0.000 (0.016) & 1.004 & & 0.000 (0.013) & 0.000 (0.013) & 1.002 & & 0.000 (0.011) & 0.000 (0.011) & 1.002 \\
$\beta$ & 1.250 & 0.105 (0.282) & -0.143 (0.096) & 2.088 & & 0.070 (0.224) & -0.163 (0.078) & 1.646 & & 0.052 (0.189) & -0.173 (0.068) & 1.376 \\
$\nu$ & 0.200 & -0.001 (0.006) & -0.001 (0.006) & 1.002 & & -0.000 (0.005) & -0.000 (0.005) & 1.002 & & -0.000 (0.004) & -0.000 (0.004) & 1.000 \\
$\alpha$ & 0.200 & 0.047 (0.140) & -0.349 (0.042) & 0.576 & & 0.032 (0.114) & -0.348 (0.033) & 0.468 & & 0.024 (0.098) & -0.348 (0.028) & 0.400 \\
\hline \hline
\end{tabular}
\end{footnotesize}
\smallskip
\begin{scriptsize}
\parbox{0.98\textwidth}{\emph{Note.} 
We simulate the process in the caption of the table 10,000 times on the interval $[0,T]$, where $T$ is interpreted as the number of days. 
There is $N = 1$ observation per unit interval, corresponding to one every day.
The true value of the parameter vector appears to the left in Panel A -- E. 
We estimate $\theta$ with the maximum composite likelihod estimation (MCLE) procedure developed in the main text, and benchmark it against a method-of-moments estimator (MME).
The table shows the Monte Carlo average of each parameter estimate across simulations (standard deviation in parenthesis).
The last column reports the RMSE ratio defined as $\text{RMSE}_{r} = \text{RMSE}( \hat{ \theta}_{ \text{MCLE}}) / \text{RMSE}( \hat{ \theta}_{ \text{MME}})$. 
}
\end{scriptsize}
\end{center}
\end{sidewaystable}


==> tables/sim-mcle-ou-q=2-N=1-mu=0.tex <==
\begin{sidewaystable}[ht!]
\setlength{ \tabcolsep}{0.15cm}
\begin{center}
\caption{Parameter estimation of the fOU process [$q = 2$ and $\mu$ known].}
\label{table:sim-ou-q=2-N=1-mu=0}
\begin{footnotesize}
\begin{tabular}{lrrrrrrrrrrrrrr}
\hline \hline
Parameter & Value & \multicolumn{3}{c}{$T = 1{,}095$} && \multicolumn{3}{c}{$T = 1{,}825$} && \multicolumn{3}{c}{$T = 2{,}555$} \\
\cline{3-5} \cline{7-9} \cline{11-13}
&& \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} && \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} && \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} \\
\hline 
Panel A: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\kappa$ & 0.005 & 0.000 (0.006) & 0.014 (0.034) & 0.160 & & 0.000 (0.004) & 0.010 (0.024) & 0.154 & & -0.000 (0.003) & 0.008 (0.020) & 0.153 \\
$\nu$ & 1.250 & -0.003 (0.033) & -0.000 (0.032) & 1.016 & & -0.002 (0.025) & -0.000 (0.025) & 1.020 & & -0.002 (0.021) & -0.001 (0.021) & 1.025 \\
$\alpha$ & -0.450 & 0.001 (0.010) & 0.004 (0.038) & 0.260 & & 0.001 (0.008) & 0.002 (0.032) & 0.240 & & 0.001 (0.006) & 0.001 (0.028) & 0.229 \\
Panel B: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\kappa$ & 0.010 & 0.002 (0.007) & 0.009 (0.024) & 0.275 & & 0.001 (0.005) & 0.006 (0.018) & 0.268 & & 0.001 (0.004) & 0.004 (0.015) & 0.266 \\
$\nu$ & 0.750 & -0.001 (0.020) & -0.001 (0.019) & 1.091 & & -0.001 (0.016) & -0.001 (0.014) & 1.090 & & -0.001 (0.013) & -0.001 (0.012) & 1.091 \\
$\alpha$ & -0.400 & 0.001 (0.015) & -0.001 (0.044) & 0.337 & & 0.001 (0.011) & -0.001 (0.035) & 0.326 & & 0.001 (0.010) & -0.000 (0.030) & 0.323 \\
Panel C: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\kappa$ & 0.015 & 0.002 (0.008) & 0.003 (0.012) & 0.628 & & 0.001 (0.006) & 0.002 (0.009) & 0.619 & & 0.001 (0.005) & 0.001 (0.008) & 0.622 \\
$\nu$ & 0.500 & -0.000 (0.015) & -0.001 (0.012) & 1.198 & & -0.000 (0.011) & -0.000 (0.009) & 1.196 & & -0.000 (0.010) & -0.000 (0.008) & 1.197 \\
$\alpha$ & -0.200 & 0.002 (0.029) & -0.002 (0.043) & 0.666 & & 0.001 (0.022) & -0.001 (0.034) & 0.659 & & 0.001 (0.019) & -0.000 (0.028) & 0.665 \\
Panel D: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\kappa$ & 0.035 & 0.004 (0.018) & 0.002 (0.015) & 1.171 & & 0.002 (0.012) & 0.001 (0.011) & 1.028 & & 0.002 (0.009) & 0.001 (0.010) & 0.975 \\
$\nu$ & 0.300 & 0.002 (0.008) & -0.001 (0.009) & 0.993 & & 0.001 (0.006) & -0.000 (0.007) & 0.889 & & 0.001 (0.005) & -0.000 (0.006) & 0.856 \\
$\alpha$ & 0.000 & 0.002 (0.043) & -0.003 (0.041) & 1.051 & & 0.001 (0.033) & -0.002 (0.032) & 1.026 & & 0.001 (0.027) & -0.001 (0.027) & 1.016 \\
Panel E: \\
$\mu$ & 0.000 & & & & & & & & & & & \\
$\kappa$ & 0.070 & 0.012 (0.040) & 0.002 (0.022) & 1.891 & & 0.009 (0.033) & 0.000 (0.017) & 2.024 & & 0.008 (0.029) & -0.000 (0.014) & 2.087 \\
$\nu$ & 0.200 & 0.011 (0.021) & -0.001 (0.009) & 2.313 & & 0.008 (0.016) & -0.001 (0.007) & 2.319 & & 0.007 (0.013) & -0.001 (0.006) & 2.273 \\
$\alpha$ & 0.200 & -0.004 (0.077) & -0.006 (0.038) & 2.021 & & -0.000 (0.067) & -0.005 (0.030) & 2.245 & & 0.002 (0.060) & -0.005 (0.025) & 2.409 \\
\hline \hline
\end{tabular}
\end{footnotesize}
\smallskip
\begin{scriptsize}
\parbox{0.98\textwidth}{\emph{Note.} 
We simulate the process in the caption of the table 10,000 times on the interval $[0,T]$, where $T$ is interpreted as the number of days. 
There is $N = 1$ observation per unit interval, corresponding to one every day.
The true value of the parameter vector appears to the left in Panel A -- E. 
We estimate $\theta$ with the maximum composite likelihod estimation (MCLE) procedure developed in the main text, and benchmark it against a method-of-moments estimator (MME).
The table shows the Monte Carlo average of each parameter estimate across simulations (standard deviation in parenthesis).
The last column reports the RMSE ratio defined as $\text{RMSE}_{r} = \text{RMSE}( \hat{ \theta}_{ \text{MCLE}}) / \text{RMSE}( \hat{ \theta}_{ \text{MME}})$. 
}
\end{scriptsize}
\end{center}
\end{sidewaystable}


==> tables/sim-mcle-ou-q=2-N=1-mu=1.tex <==
\begin{sidewaystable}[ht!]
\setlength{ \tabcolsep}{0.15cm}
\begin{center}
\caption{Parameter estimation of the fOU process [$q = 2$ and $\mu$ estimated].}
\label{table:sim-ou-q=2-N=1-mu=1}
\begin{footnotesize}
\begin{tabular}{lrrrrrrrrrrrrrr}
\hline \hline
Parameter & Value & \multicolumn{3}{c}{$T = 1{,}095$} && \multicolumn{3}{c}{$T = 1{,}825$} && \multicolumn{3}{c}{$T = 2{,}555$} \\
\cline{3-5} \cline{7-9} \cline{11-13}
&& \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} && \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} && \multicolumn{1}{c}{MCLE} & \multicolumn{1}{c}{MME} & \multicolumn{1}{c}{RMSE$_{r}$} \\
\hline 
Panel A: \\
$\mu$ & 0.000 & 0.001 (0.255) & 0.001 (0.258) & 0.987 & & -0.002 (0.161) & -0.002 (0.164) & 0.983 & & -0.001 (0.118) & -0.001 (0.120) & 0.982 \\
$\kappa$ & 0.005 & 0.002 (0.007) & 0.017 (0.037) & 0.177 & & 0.001 (0.004) & 0.011 (0.026) & 0.160 & & 0.000 (0.003) & 0.009 (0.021) & 0.157 \\
$\nu$ & 1.250 & -0.003 (0.033) & -0.000 (0.032) & 1.016 & & -0.002 (0.025) & -0.000 (0.025) & 1.019 & & -0.002 (0.021) & -0.001 (0.021) & 1.022 \\
$\alpha$ & -0.450 & 0.002 (0.010) & 0.004 (0.038) & 0.264 & & 0.001 (0.008) & 0.002 (0.032) & 0.242 & & 0.001 (0.006) & 0.001 (0.028) & 0.230 \\
Panel B: \\
$\mu$ & 0.000 & 0.001 (0.093) & 0.001 (0.094) & 0.996 & & -0.000 (0.061) & -0.000 (0.061) & 0.992 & & -0.000 (0.046) & -0.000 (0.046) & 0.991 \\
$\kappa$ & 0.010 & 0.003 (0.007) & 0.010 (0.025) & 0.294 & & 0.001 (0.005) & 0.006 (0.018) & 0.277 & & 0.001 (0.004) & 0.005 (0.015) & 0.271 \\
$\nu$ & 0.750 & -0.002 (0.020) & -0.001 (0.019) & 1.083 & & -0.001 (0.016) & -0.001 (0.014) & 1.082 & & -0.001 (0.013) & -0.001 (0.012) & 1.085 \\
$\alpha$ & -0.400 & 0.002 (0.015) & -0.001 (0.045) & 0.338 & & 0.001 (0.012) & -0.001 (0.035) & 0.327 & & 0.001 (0.010) & -0.000 (0.030) & 0.324 \\
Panel C: \\
$\mu$ & 0.000 & 0.002 (0.098) & 0.002 (0.097) & 1.007 & & 0.000 (0.070) & 0.000 (0.069) & 1.003 & & 0.000 (0.055) & 0.000 (0.055) & 1.002 \\
$\kappa$ & 0.015 & 0.004 (0.009) & 0.004 (0.013) & 0.677 & & 0.002 (0.006) & 0.002 (0.010) & 0.643 & & 0.002 (0.005) & 0.002 (0.008) & 0.636 \\
$\nu$ & 0.500 & -0.001 (0.014) & -0.001 (0.012) & 1.174 & & -0.001 (0.011) & -0.000 (0.009) & 1.185 & & -0.000 (0.009) & -0.000 (0.008) & 1.186 \\
$\alpha$ & -0.200 & 0.005 (0.029) & -0.002 (0.044) & 0.670 & & 0.003 (0.022) & -0.001 (0.034) & 0.662 & & 0.002 (0.019) & -0.000 (0.028) & 0.664 \\
Panel D: \\
$\mu$ & 0.000 & 0.001 (0.068) & 0.001 (0.067) & 1.007 & & -0.000 (0.053) & -0.000 (0.052) & 1.004 & & 0.000 (0.044) & 0.000 (0.044) & 1.003 \\
$\kappa$ & 0.035 & 0.008 (0.017) & 0.004 (0.016) & 1.154 & & 0.005 (0.012) & 0.002 (0.012) & 1.020 & & 0.003 (0.009) & 0.002 (0.010) & 0.991 \\
$\nu$ & 0.300 & 0.002 (0.008) & -0.000 (0.009) & 0.989 & & 0.001 (0.006) & -0.000 (0.007) & 0.887 & & 0.001 (0.005) & -0.000 (0.006) & 0.861 \\
$\alpha$ & 0.000 & 0.008 (0.041) & -0.002 (0.041) & 1.007 & & 0.005 (0.032) & -0.002 (0.032) & 0.992 & & 0.004 (0.027) & -0.001 (0.027) & 0.998 \\
Panel E: \\
$\mu$ & 0.000 & 0.001 (0.069) & 0.001 (0.068) & 1.005 & & -0.000 (0.059) & -0.000 (0.059) & 1.003 & & -0.000 (0.053) & -0.000 (0.053) & 1.002 \\
$\kappa$ & 0.070 & 0.010 (0.029) & 0.007 (0.022) & 1.296 & & 0.007 (0.024) & 0.004 (0.017) & 1.443 & & 0.006 (0.021) & 0.003 (0.014) & 1.524 \\
$\nu$ & 0.200 & 0.011 (0.014) & -0.001 (0.010) & 1.674 & & 0.008 (0.011) & -0.001 (0.007) & 1.713 & & 0.006 (0.010) & -0.001 (0.006) & 1.727 \\
$\alpha$ & 0.200 & -0.019 (0.055) & -0.006 (0.038) & 1.479 & & -0.013 (0.049) & -0.005 (0.030) & 1.658 & & -0.009 (0.045) & -0.005 (0.025) & 1.809 \\
\hline \hline
\end{tabular}
\end{footnotesize}
\smallskip
\begin{scriptsize}
\parbox{0.98\textwidth}{\emph{Note.} 
We simulate the process in the caption of the table 10,000 times on the interval $[0,T]$, where $T$ is interpreted as the number of days. 
There is $N = 1$ observation per unit interval, corresponding to one every day.
The true value of the parameter vector appears to the left in Panel A -- E. 
We estimate $\theta$ with the maximum composite likelihod estimation (MCLE) procedure developed in the main text, and benchmark it against a method-of-moments estimator (MME).
The table shows the Monte Carlo average of each parameter estimate across simulations (standard deviation in parenthesis).
The last column reports the RMSE ratio defined as $\text{RMSE}_{r} = \text{RMSE}( \hat{ \theta}_{ \text{MCLE}}) / \text{RMSE}( \hat{ \theta}_{ \text{MME}})$. 
}
\end{scriptsize}
\end{center}
\end{sidewaystable}

